Snowmass White Paper: Precision Studies of Spacetime Symmetries and Gravitational Physics

High-energy physics is primarily concerned with uncovering the laws and principles that govern nature at the fundamental level. Research in this field usually relies on probing the boundaries of established physics, an undertaking typically associated with extreme energy and distance scales. It is therefore unsurprising that particle physics has traditionally been dominated by large-scale experimental methods often involving high energies, such as colliders and storage rings, cosmological and astrophysical observations, large-volume detector systems, etc. However, high-sensitivity measurements in smaller experiments, often performed at lower energies, are presently experiencing a surge in importance for particle physics for at least two reasons. First, they exploit synergies to adjacent areas of physics with recent advances in experimental techniques and technology. Together with intensified phenomenological explorations, these advances have led to the realization that challenges associated with weak couplings or the expected suppression factors for new physics can be overcome with such methods while maintaining a large degree of experimental control. Second, many of these measurements broaden the range of particle-physics phenomena and observables relative to the above set of more conventional methodologies. Combining such measurements with the conventional efforts above therefore casts both a wider and tighter net for possible effects originating from physics beyond the Standard Model (BSM). This paper argues that this assessment points at a growing impact of such methods and measurements on high-energy physics, and therefore warrants direct support as particle-physics research. Leveraging the recent rapid progress and bright outlook associated with such studies for high-energy physics, could yield high returns, but requires substantial and sustained efforts by funding agencies.

==> muGrav/Snowmass2021-MuGrav-LoI-RF0-AF0-005-text.tex <==
\section{Introduction}\vspace{-.05in}
\label{intro}
The question of antimatter gravity, first raised in the 1950s~\cite{Morrison}, is of continuing interest~\cite{Nieto-Goldman,Fischler-Lykken-Roberts}. In the (perhaps counterintuitive, and controversial) ``antigravity" scenario, antimatter is predicted to repel matter~\cite{Morrison,Kowitt,Kerr-Newman1,Blanchet-LeTiec-2008,Kerr-Newman3,Blanchet-LeTiec-2009,Cabbolet,Hajdukovic-2011,Villata-2011,BenoitLevy-Chardin,Hajdukovic-2012,Villata-2012,Villata-2013,Kerr-Newman5}, potentially solving several problems in cosmology~\cite{MAGE-Atoms}; while in a field-theory-motivated framework, the gravitational acceleration of antimatter by matter could differ slightly from that of matter~\cite{Nieto-Goldman}, contrary to expectations from general relativity, and perhaps provide clues to the correct quantum theory of gravity. %To~date, 
Decades of experimental effort
have yet to yield a statistically significant direct measurement. Antimatter gravity studies using antihydrogen (${\overline {\rm H}}$) are ongoing~\cite{ALPHA,AEGIS,AEGIS2,gbar}, and experiments with positronium have been discussed~\cite{Cassidy-Hogan}. 
We here consider a possible measurement with muonium (M or Mu), an~exotic atom consisting of an electron bound to an antimuon; unlike the ${\overline {\rm H}}$ case, the interpretation of such a measurement  has no hadronic uncertainties. This measurement\,---\,the goal of the Muonium Antimatter Gravity Experiment (MAGE) collaboration\,---\,could potentially be performed at an upgraded Fermilab muon complex~\cite{muonLoI}.


The most sensitive ($\sim10^{-7}$) limits on antimatter gravity  come from {\em indirect} tests  (for example, equivalence principle tests using torsion pendula~\cite{EotWash} or masses in Earth orbit~\cite{MICROSCOPE}), relying on the expected amounts of virtual antimatter in the nuclei of various elements~\cite{Alves}; these are invalid in the antigravity scenario and, in any case, are inapplicable to muonium. Another limit,  $|\alpha_g-1|<8.7\times10^{-7}$~\cite{Ulmer}, has been derived from the measured cyclotron frequency of magnetically confined antiprotons, compared with that of H$^-$ ions, based on the gravitational redshift due to Earth's gravitational potential in the field of the local galactic supercluster~\cite{Hughes,Gabrielse-1990,Good}; it too need not apply to antimuons.\footnote{And we note that arguments based on absolute gravitational potentials have been critiqued by Nieto and Goldman~\cite{Nieto-Goldman}. Other precise measurements of these cyclotron frequencies~\cite{ATRAP-1999,BASE-2017} have not been interpreted in terms of possible matter--antimatter gravitational differences.} A {\em direct} test of the gravitational interaction of antimatter with matter is desirable on quite general grounds~\cite{Nieto-Goldman}.\footnote{The only published direct test so far~\cite{ALPHA} has yielded the limit  $-65 < \gbar/g < 110$.} Such a measurement can be viewed as a test of general relativity
or as a search for a fifth force and is of interest from both perspectives.

\vspace{-.1in}\section{Experiment Concept}\vspace{-.05in}

A direct test of antimatter gravity can be performed interferometrically, by passing an intense, high-quality muonium beam in vacuum through precise nanofabricated gratings and measuring the gravity-induced phase shift~\cite{MAGE-Atoms,Kirch-Khaw,Kirch-2007}.  As shown in Fig.~\ref{fig:MAGE-concept},  a horizontal, parallel, slow muonium beam impinges on  a 3-grating, Mach--Zehnder-type interferometer, with the interference pattern following the beam's gravitational  acceleration. Mu atoms  decaying after the third grating are detected as a coincidence between a fast positron in the barrel detector and a slow electron electrostatically accelerated onto a microchannel plate at the back. The interferometric phase is measured by translating a grating continually up and down and analyzing the resulting changes in detected coincidence rate. The phase is quite small: $\Delta\phi = 2\pi \gbar t^2/d\approx 0.01$ (for $\gbar = g$), where $t$ is the time for the atom to traverse the distance between gratings and $d$ is the grating pitch (here taken as 100\,nm). The required few-picometer alignment system is feasible using laser interferometry~\cite{MAGE-Atoms,TFG-JINST,Thapa-etal}. The zero-deflection phase is determined by periodically illuminating the interferometer with soft X-rays, with a systematic check provided  by periodically rotating the interferometer by 90 or 180$^\circ$.

\begin{figure}[tb]
  \begin{minipage}[c]{0.42\textwidth}
    \caption{
MAGE experiment concept (elevation view; gravitational deflection and phase shift $\Delta\phi$ exaggerated for clarity). Muonium beam enters from left, slow-electron detector is at right. Not shown: ring electrodes to accelerate slow electrons onto their detector, starting downstream of grating 3 and continuing within scintillating-fiber-barrel positron detector;  hodoscope around positron barrel.}\label{fig:MAGE-concept}
  \end{minipage}\vspace{-.2in}
  \begin{minipage}[c]{0.57\textwidth}\vspace{-.15in}
    \includegraphics[width=\textwidth]{MAGE-concept}
  \end{minipage}%\vspace{-.1in}
\end{figure}

Preparing the intense, high-quality Mu beam needed for MAGE is a challenge. Beam R\&D is currently carried out at Switzerland's Paul Scherrer Institute (PSI)~\cite{muCool} following ideas of Taqqu~\cite{Taqqu-Proc,Taqqu-PRL}, involving cooling of a surface muon beam in  gaseous helium in crossed electric and magnetic fields to reduce its 6D emittance by some 10 orders of magnitude, at a cost of two to three orders of magnitude in muon decay loss. The cooled beam can then be stopped in a $\sim\mu$m-thick layer of superfluid helium (SFHe) at the bottom of a cryostat, efficiently forming muonium, which is then expelled vertically from the upper SFHe surface at a predicted speed of 6.3\,mm/$\mu$s~\cite{Taqqu-PRL} due to its large, positive chemical potential (270\,K) in SFHe~\cite{Taqqu-Proc}. The vertical beam is turned to  horizontal, as needed for MAGE, by means of a 45$^\circ$\ SFHe-coated deflector~\cite{SFHe-Lens}. (Because the Mu
atoms are in thermal equilibrium with the SFHe prior to expulsion, both the  beam energy spread
and its angular divergence  are determined by the ratio of the $\sim 0.2$\,K SFHe temperature to the Mu chemical potential.) The resulting interferometer acceptance is maximal,
leading to a  $5\sigma$ \gbar\ sign determination  with about one month's worth of beam at PSI~\cite{MAGE-Atoms}.

Another beam option exploits  another idea of Taqqu's~\cite{Taqqu-Proc}: use a 100-times-thicker SFHe layer, thus needing no muon cooling, so potentially providing two orders of magnitude higher intensity than the ``muCool" beam discussed above; it could be developed at Fermilab in parallel to the work in progress at PSI. This ``thick-film" approach could enable a $\stackrel{<}{_\sim}$\,$10$\% measurement of \gbar\ in a month of beam time at PSI~\cite{MAGE-Atoms}, and potentially a 1\% or higher-precision measurement at a future Fermilab facility. Since only Mu atoms formed close to the upper SFHe surface will emerge upwards to form the desired beam, an electric field is maintained in the helium (via a pool of negative charge at the SFHe surface) to cause the stopping $\mu^+$ to separate from their ionization trails and drift to the upper surface before forming Mu. %Some deadtime may be incurred if the pool of charge needs to be periodically replenished (e.g., via a submerged emitter tip). 
The $\sim$\,cm-wide beam results in some acceptance loss if cm-wide gratings are employed, thus larger gratings (if feasible) could be beneficial; alternatively, the SFHe deflector could have a curved surface so as to produce some focusing of the beam into the interferometer~\cite{SFHe-Lens}.

Surface muon beams, available at J-PARC and MuSIC in Japan, ISIS in the U.K., TRIUMF in Canada, and PSI, are currently unavailable in the U.S. As the record holder for surface-muon beam intensity, PSI\,---\,with up to $\sim$\,$10^9$\,Hz surface-muon rate, and an upgrade to $10^{10}$ under discussion, to be produced using $\sim$\,$10^{12}$\,Hz of 590\,MeV protons on target\,---\,has been the natural venue for muonium-beam R\&D.
With potentially $\stackrel{>}{_\sim}$\,$10^{13}$\,Hz of protons on target, the coming PIP-II intensity upgrade~\cite{PIP-II} could make Fermilab the world leader for both fundamental muon experiments and the Muon Spin Rotation community~\cite{LEmuon-LoI};  %upgrade is under discussion with the goal of producing $\sim$\,$10^{10}$\,Hz of surface muons. This requires $\sim$\,$10^{12}$\,Hz of protons on target (depending on beam energy and target configuration), so an intensity in this ballpark is required in order to be competitive. To obtain a more precise estimate will require a study of the trade-offs among beam energy and target material, length, and geometry. 
 the novel muonium beams discussed above could be used as-is for MAGE~\cite{MAGE-Atoms} and other muonium experiments, or ionized to serve %world-leading 
muon experiments~\cite{Mu-g-2}.  


%[ADD A BIT MORE DETAIL?]

\vspace{-.1in}
\section{R\&D}\vspace{-.05in}

To enhance  beam design progress in the interim period before a new facility can be built, an R\&D platform would be extremely useful and, for some applications (e.g., SFHe Mu production), even crucial. This could be provided at  the Fermilab ``MuCool Test Area" (MTA)~\cite{Johnstone-Johnstone}, or (at lower intensity) using the Fermilab Test Beam Facility (FTBF). Other options may also be available.

\vspace{-.1in}
\section{Conclusion}\vspace{-.05in}

We propose to study the options for providing competitive muonium beams at Fermilab in the Mu2e and PIP-II ``eras." This study can inform  proposals for MAGE at Fermilab as well as other future experiments employing muonium, such as the precision determination of the  hyperfine and 1S--2S transition frequencies~\cite{Gorringe-Hertzog,Crivelli,Mills}, the search for Mu--$\overline{\rm Mu}$ oscillation~\cite{Jungmann}, etc.

%\hfill\eject

\begin{thebibliography}{99}
\bibitem{Morrison}
P. Morrison, 
``Approximate Nature of Physical Symmetries,"
 Am.\ J. Phys.\ {\bf 26}, 358, (1958).

\bibitem{Nieto-Goldman}
M. M. Nieto, T. Goldman, 
``The Arguments Against `Antigravity' and the Gravitational Acceleration of Antimatter," {Phys.\ Rep.}\ {{\bf 205}, 221--281 (1991)}.

\bibitem{Fischler-Lykken-Roberts}
M. Fischler, J. Lykken, T. Roberts, ``Direct Observation Limits on Antimatter Gravitation," Tech.\ Rep.\  FERMILAB-FN-0822-CD-T. 2008. Available online: \url{http://arxiv.org/abs/0808.3929}.
%\textcolor{red}{( please add the date.)}

\bibitem{Kowitt}
M. Kowitt, ``Gravitational repulsion and Dirac antimatter," {Int.\ J. Theor.\ Phys.}\ {\bf 35} (1996) 605--631.


%28--33
\bibitem{Blanchet-LeTiec-2008}
 L. Blanchet, A. Le Tiec, ``Model of dark matter and dark energy based on gravitational polarization," {Phys.~Rev.~D}  {\bf 78}, 024031 (2008).

%29--34
%\bibitem{Burinskii}
%\hl{Burinskii,  A. The Dirac-Kerr-Newman electron.}  {\em Gravit.\ Cosmol.}\ {\bf 2008}, {\em 14}, 109--122.


 %30--35
\bibitem{Blanchet-LeTiec-2009}
 L. Blanchet, A. Le Tiec, ``Dipolar dark matter and dark energy,"  {Phys.\ Rev.\ D}  {\bf 80}, 023524 (2009).


%31--36
\bibitem{Cabbolet}
M.J.T.F. Cabbolet,  ``Elementary Process Theory: A formal axiomatic system with a potential application as a foundational framework for physics supporting gravitational repulsion of matter and antimatter," {Ann.\ Phys.}\ {\bf 522}, 699--738 (2010).


%32--37
\bibitem{Hajdukovic-2011}
D.S. Hajdukovic, ``Is dark matter an illusion created by the gravitational polarization of the quantum vacuum?,"  {Astrophys.\ Space Sci.}\  {\bf 334}, 215--218 (2011).

%33--38
\bibitem{Villata-2011}
M. Villata,``CPT symmetry and antimatter gravity in general relativity,"
  {Europhys.\ Lett.}\  {\bf 94} (2011) 20001.

%34--39
\bibitem{BenoitLevy-Chardin}
A.  Benoit-L\'evy, G. Chardin, ``Introducing the Dirac--Milne universe,"
 {Astron.\ Astrophys.}\  {\bf 537}, A78 (2012).

 %35--40
\bibitem{Hajdukovic-2012}
 D. Hajdukovic, ``Quantum vacuum and virtual gravitational dipoles: the solution to the dark energy problem?,"  {Astrophys.\ Space Sci.}\  {\bf 339}, 1--5 (2012).

 %36--41
\bibitem{Villata-2012}
M. Villata,  ``\,`Dark energy' in the Local Void," {Astrophys.\ Space Sci.}\  {\bf  339}, 7--12 (2012).

 %37--42
\bibitem{Villata-2013}
 M. Villata,  ``On the nature of dark energy: The lattice Universe,"  {Astrophys.\ Space Sci.}\  {\bf  345}, 1--9 (2013).
 
 \bibitem{Kerr-Newman1}
G. Chardin, ``Motivations for antigravity in general relativity," {Hyperfine\ Int.}\ {\bf 109}, 83--94 (1997).

%\bibitem{Kerr-Newman2}
%Arcos,  H.I.; Pereira,  J.G. Kerr-Newman solution as a Dirac particle. {\em Gen.\ Rel.\ Grav.}\ {\bf 2004}, {\em 36}, 2441--2464.

%50--29
\bibitem{Kerr-Newman3}
 A. Burinskii, ``The Dirac--Kerr--Newman electron," {Gravit.\ Cosmol.} {\bf  14}, 109--122 (2008).
%\textcolor{red}{(reference 29 is as same as the reference 34, please confirm.)}

 %51--30

 \bibitem{Kerr-Newman5}
M. Villata, ``The matter--antimatter interpretation of Kerr spacetime," Ann.\ Phys.\ (Berl.)\ {\bf 527}, 507 (2015).
 
 \bibitem{MAGE-Atoms}
A. Antognini {\it et al.}, ``Studying Antimatter Gravity with Muonium," Atoms {\bf 6,} 17 (2018); \url{doi:10.3390/atoms6020017}.

\bibitem{ALPHA}
C. Amole {\it et al.},
``Description and first application of a new technique to measure the gravitational mass of antihydrogen," {Nat.\ Commun.}\ {\bf 4}, 1--9  {(2013)}.


\bibitem{AEGIS}
A. Kellerbauer {\it et al.},
``Probing antimatter gravity---The AEGIS experiment at CERN,"
In~Proc.\ 4th Int.\ Conf.\ on New Frontiers in Physics  (ICNFP 2015), Crete, Greece, 23--30 August 2015, ed.\ L. Bravina, Y. Foka, S. Kabana,  EPJ Web of Conf. EDP Sciences: Les Ulis, France, 2016; Volume  126, p. 02016. %\textcolor{red}{( please provide the publisher and location.)}


\bibitem{AEGIS2}
G. Drobychev {\it et al.},
Proposal for the AEGIS Experiment at the CERN Antiproton Decelerator, Tech.\ Rep.\ CERN-SPSC-2007-017, CERN, June 2007. Available online: \url{http://doc.cern.ch//archive/electronic/cern/preprints/spsc/public/spsc-2007-017.pdf}.
%please add the date
%we deleted `(AEGIS Collaboration)', please confirm

\bibitem{gbar}
P. Perez, Y. Sacquin,
``The GBAR experiment: gravitational behaviour of antihydrogen at rest,"
{Class.\ Quantum Gravity} {\bf 29}, 184008 {(2012)}.

\bibitem{Cassidy-Hogan}
D. B. Cassidy, S. D. Hogan, 
``Atom control and gravity measurements using Rydberg positronium," {Int.\ J. Mod.\ Phys. Conf.\ Ser.}\  {\bf  30}, 1460259 (2014).

 \bibitem{muonLoI}
R. H. Bernstein {\it et al.}, ``Letter of Interest for an Upgraded Low-Energy Muon Facility at Fermilab," submission to Snowmass 2021 (2020), \url{https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF0-AF0-007.pdf}.


\bibitem{EotWash}
T. A. Wagner, S. Schlamminger, J. H. Gundlach, E. G.  Adelberger,
``Torsion-balance tests of the weak equivalence principle," {Class.\ Quantum Gravity}  {\bf 29},
184002 {(2012)}.

\bibitem{MICROSCOPE}
P. Touboul {\it et al.},
``The MICROSCOPE mission: First results of a space test of the Equivalence Principle," {Phys.~Rev. Lett.}\  {\bf 119}, 231101 {(2017)}.


\bibitem{Alves}
D. S. M. Alves, M. Jankowiak, P. Saraswat,
``Experimental constraints on the free fall acceleration of antimatter," arXiv:0907.4110 (2009).


\bibitem{Ulmer}
S. Ulmer {\it et al.},  ``High-precision comparison of the antiproton-to-proton charge-to-mass ratio," {Nature} {\bf 524}, 196--199 (2015).


\bibitem{Hughes}
R. J. Hughes, M. H. Holzscheiter, ``Constraints on the gravitational properties of
antiprotons and positrons from cyclotron-frequency measurements," {Phys. Rev. Lett.}\ {\bf 66}, 854--857 (1991).

\bibitem{Gabrielse-1990}
G. Gabrielse {\it et al.}, ``Thousandfold Improvement in the Measured Antiproton Mass," {Phys.\ Rev.\ Lett.}\ {\bf 65}, 1317--1320, (1990).

\bibitem{Good}
M. L. Good, ``$K_2^0$
 and the Equivalence Principle," Phys. Rev.  {\bf 121}, 311 (1961).

\bibitem{Kirch-Khaw}
K. Kirch and K. S. Khaw, Int.\ J. Mod.\ Phys.\ Conf.\ Ser.\ {\bf 30}, 1460258 (2014), Proc.\ 2nd Int.\ Workshop Antimatter and Gravity (WAG2013); arXiv:1509.02918.

\bibitem{Kirch-2007}
K. Kirch, ``Testing Gravity with Muonium,"
 arXiv:physics/0702143 [physics.atom-ph] (2008).
 
 \bibitem{TFG-JINST}
D. M. Kaplan, T. J. Roberts, J. D Phillips, R. D. Reasenberg, ``Improved performance of seminconductor laser tracking frequency gauge," JINST {\bf 13} (2018) P03008.

\bibitem{Thapa-etal}
R. Thapa, J. D. Phillips, E. Rocco, R. D. Reasenberg,  ``Subpicometer length measurement using semiconductor laser tracking frequency gauge," {Opt.\ Lett.}\ {\bf 36}, 3759--3761 (2011).

\bibitem{muCool}
A. Antognini {\it et al.}, ``Demonstration of Muon-Beam Transverse Phase-Space Compression," arXiv:    2003.11986 [physics.acc-ph] (2020);\\
R. Iwai {\it et al.}, ``Development of next generation muon beams at the Paul Scherrer Institute," Proc. 21st Int. Workshop on Neutrinos from Accelerators (Nufact19), PoS NuFact2019 (2020) 125; DOI:
10.22323/1.369.0125

\bibitem{Taqqu-Proc}
D. Taqqu, ``Ultraslow Muonium for a Muon beam of ultra high quality," Phys.\ Procedia {\bf 17} (2011) 216.
\bibitem{Taqqu-PRL}
D. Taqqu, ``Compression and Extraction of Stopped Muons," Phys.\ Rev.\ Lett.\ {\bf 97} (2006) 194801.


\bibitem{ATRAP-1999}
G. Gabrielse {\it et al.}, ``Precision Mass Spectroscopy of the Antiproton and Proton Using Simultaneously Trapped Particles,"
Phys. Rev. Lett.\ {\bf 82},  3198 (1999).

\bibitem{BASE-2017}
C. Smorra {\it et al.}, ``A parts-per-billion measurement of the antiproton magnetic moment," {Nature}   {\bf 550}, 371--374 (2017).

\bibitem{SFHe-Lens}
V. G. Luppov {\it et al.}, ``Focusing a Beam of Ultracold Spin-Polarized Hydrogen Atoms with a Helium-Film-Coated Quasiparabolic Mirror," Phys. Rev. Lett. {\bf 71}, 2405 (1993).
 
%\bibitem{DeGouvea-Vogel}
%A. De Gouv\^{e}a, P. Vogel, Prog.\ Part.\ Nucl.\ Phys.\ {\bf 71}, 75 (2013); arXiv:1303.4097 [hep-ph].
%\bibitem{Iinuma}
%H. Iinuma, J. Phys.\ Conf.\ Ser.\ {\bf 295}, 012032 (2011).
%\bibitem{Adelmann}
%A. Adelmann, K. Kirch, C. J. G. Onderwater, and
%T. Schietinger, J. Phys.\ G Nucl.\ Part.\ Phys.\ {\bf 37}, 085001 (2010).
%\bibitem{Crivellin}
%A. Crivellin, M. Hoferichter, and P. Schmidt-Wellenburg, Phys.\ Rev.\ D {\bf 98}, 113002 (2018).
%\bibitem{Bernstein-Cooper}
%R. H. Bernstein, P. S. Cooper, Phys.\ Rep.\ {\bf 532}, 27 (2013);  \url{https://doi.org/10.1016/j.physrep.2013.07.002}.
%\bibitem{Jungmann}
%K. Jungmann, ``Muonium - Physics of a most Fundamental Atom," Nucl.\ Phys.\ B (Proc.\ Suppl.)\ {\bf 155} (2006) 355.

%\bibitem{SEEMS}
%See \url{https://www.ornl.gov/event/opportunities-seems-facility} and \url{https://traviswilliams.ornl.gov/seems/} (accessed 5/13/2020).

\bibitem{PIP-II}
V. Shiltsev, ``Fermilab Proton Accelerator Complex Status and Improvement Plans," Mod.\ Phys.\ Lett.\ A {\bf 32}  (2017) 1730012; FERMILAB-PUB-017-129-APC (2017).
%\bibitem{ES-PSI}
%K. Kirch {et al.} (eds.), Particle Physics and Related Topics at the Paul Scherrer Institute: Input to the European Strategy process, \url{https://indico.cern.ch/event/765096/contributions/}, No.\ 121.
%\bibitem{Kirch-piE5}
%K. Kirch, private communication.
%\bibitem{Prokscha-etal}
%T. Prokscha {\it et al.}, ``The new $\mu$E4  beam at PSI: A hybrid-type large acceptance channel for the generation of a high intensity surface-muon beam," Nucl.\ Instrum.\ Meth.\ A {\bf 595} (2008) 317, \url{https://doi.org/10.1016/j.nima.2008.07.081}.
%\bibitem{TRIUMF}
%``Muon Beamlines at TRIUMF," web page, \url{http://cmms.triumf.ca/equip/mubeamlines/node1.html#tabbeamlines} (accessed 4/21/2020).
%\bibitem{Hino-etal}
%Y. Hino {\it et al.}, ``A Highly intense DC muon source, MuSIC and muon CLFV search," Nucl.\ Phys.\ B Proc.\ Suppl.\ {\bf 253--255} (2014) 206, XII Int.\ Workshop on Tau-Lepton Phys.\ (TAU2012). ; \url{https://doi.org/10.1016/j.nuclphysbps.2014.09.051}.
%\bibitem{Kawamura}
%N. Kawamura, ``Muon beamlines and Target Technologies at J-PARC," presented at Compact muon sources workshop, Univ.\ of Huddersfield, 12--13 Jan.\ 2015, \url{https://indico.cern.ch/event/356972/contributions/1766762/attachments/710282/975044/FutureMuonSources_20150112.pptx} (accessed 4/21/2020). 
%\bibitem{Mu2eTDR}
%Mu2e Document 4299-v15: Mu2e Technical Design Report (TDR), Ch.\ 4 Accelerators, available from https://mu2e-docdb.fnal.gov/cgi-bin/ShowDocument?docid=4299 (accessed 4/28/2020).
%\bibitem{Renga-etal}
%F. Renga, G. Cavoto, A. Papa, E. Ripiccini, C. Voena, ``The Quest for $\mu\to e\gamma$ and its Experimental Limiting Factors at Future High Intensity Muon Beams," arXiv:1811.12324 [hep-ex] (2018).
%G. Cavoto, A. Papa, F. Renga, E. Ripiccini, C. Voena, ``The quest for $\mu\to e\gamma$ and its experimental limiting factors at future high intensity muon beams," Eur.\ Phys.\ J. C {\bf 78}  (2018) 37; arXiv:1811.12324 [hep-ex] (2018).
%\bibitem{Cheng-Echenard-Hitlin}
%C.-h. Cheng, B. Echenard, D. Hitlin, ``The next generation of $\mu\to e\gamma$ and $\mu\to  3e$ CLFV search experiments," arXiv:1309.7679 [physics.ins-det] (2013).
%\bibitem{Pronskikh-etal}
%V. S. Pronskikh {\it et al.}, ``Target Station Design for the Mu2e Experiment," Proc.\ IPAC2014, paper THPRI085 (2014).

\bibitem{LEmuon-LoI}
R. H. Bernstein {\it et al.}, Letter of Interest for a Muonium Gravity Experiment at Fermilab, submitted to Snowmass 2021 Workshop, \url{https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF0-AF0-007.pdf}.

\bibitem{Mu-g-2}
%Conceptual design report for the measurement of the muon anomalous magnetic moment $g- 2$ and electric dipole moment at J-PARC. Technical report, J-PARC, 2011. Available from \url{https://g2sakura.kek.jp/public/doc/MCDR-submit.pdf}.
S. Kanda, ``Muonium production target for the muon $g-2$/EDM experiment at J-PARC," Nucl.\ Phys.\ B Proc.\ Supp\.\ {\bf 253} 212 (2014), XII Int.\ Workshop on Tau-Lepton Phys.\ (TAU2012); \url{https://doi.org/10.1016/j.nuclphysbps.2014.09.054}.

\bibitem{Johnstone-Johnstone}
A more ambitious scheme for a muon beam in the MTA is discussed in J. A. Johnstone, C. Johnstone, ``Prospects for a Muon Spin Resonance Facility in the Fermilab Mucool Test Area," Proc. IPAC2018, paper MOPML032 (2018).

\bibitem{Gorringe-Hertzog}
T. Gorringe and D. Hertzog, ``Precision Muon Physics," Prog.\ Part.\ Nucl.\ Phys.\ {\bf 84}, 73 (2015).

\bibitem{Crivelli}
P. Crivelli, ``The Mu-MASS (MuoniuM lAser SpectroScopy) experiment," Hyperfine Interact.\ {\bf 239}, 49 (2018).

\bibitem{Mills}
A. P. Mills, ``Precision Experiments with Ultraslow Muons," Proc.\ Int.\ Symp.\ Sci.\ Explored by Ultra Slow Muon (USM2013),
JPS Conf. Proc. {\bf 2,} 010401 (2014).

\bibitem{Jungmann}
K. P. Jungmann, ``Precision Muonium Spectroscopy," J. Phys.\ Soc.\ Japan {\bf 85}, 091004 (2016).

\end{thebibliography}
%\end{document}
